Gravitational Wave Data Analysis: Computing Challenges in the 3G Era

Cyber infrastructure will be a critical consideration in the development of next generation gravitational-wave detectors. The demand for data analysis computing in the 3G era will be driven by the high number of detections as well as the expanded search parameter space for compact astrophysical objects and the subsequent parameter estimation follow-up required to extract the nature of the sources. Additionally, there will be an increased need to develop appropriate and scalable computing cyberinfrastructure, including data access and transfer protocols, and storage and management of software tools, that have sustainable development, support, and management processes. This report identifies the major challenges and opportunities facing 3G gravitational-wave observatories and presents recommendations for addressing them. This report is the fourth in a six part series of reports by the GWIC 3G Subcommittee: i) Expanding the Reach of Gravitational Wave Observatories to the Edge of the Universe, ii) The Next Generation Global Gravitational Wave Observatory: The Science Book, iii) 3G R&D: R&D for the Next Generation of Ground-based Gravitational Wave Detectors, iv) Gravitational Wave Data Analysis: Computing Challenges in the 3G Era (this report), v) Future Ground-based Gravitational-wave Observatories: Synergies with Other Scientific Communities, and vi) An Exploration of Possible Governance Models for the Future Global Gravitational-Wave Observatory Network.

==> acronyms.tex <==
\chapterimage{figures/bbh} % Chapter heading image
\chapter*{Acronyms \& abbreviations}
\addcontentsline{toc}{chapter}{\color{ocre} Acronyms and Abbreviations}
\begin{table}[h!]
\parbox{1.0\linewidth}{
\begin{tcolorbox}[standard jigsaw,colframe=ocre,colback=ocre!10!white,opacityback=0.6,coltext=black,title=\sc \large Acronyms and abbreviations used in the text]
\small
%\caption{}
\vskip-5pt
\label{tab:acronyms}
\parbox{.50\linewidth}{
	\begin{tabular}{rl}
	%\hline
	%\hline
	%{\bf Abbreviation} & {\bf Definition } \\
        % \hline 
	3G	& \emph{Third-generation}, the next generation of ground-based gravitational-wave observatories \\
	    & \emph consisting of 1 ET in Europe, 1 CE each in the US and Australia\\
	BAO	& \emph{Baryon Acoustic Oscillations} \\
	BBH	& \emph{Binary Black Hole}, a binary system of two black holes \\
	BH	& \emph{Black Hole}\\
	BNS	& \emph{Binary Neutron Star}, a binary system of two neutron stars\\
	CE	& \emph{Cosmic Explorer}, concept for a US third generation interferometer with 40 km arms \\
	CMB	& \emph{Cosmic Microwave Background} \\
	ECO	& \emph{Exotic Compact Object}, an alternative to a neutron star or a black hole \\
	EM	& \emph{Electromagnetic} \\
	ET	& \emph{Einstein Telescope}, concept for a European triangular shaped interferometer with 10 km arms\\
	GR	& \emph{General relativity} \\
	GSF	& \emph{Gravitational Self-Force} \\
	GW	& \emph{Gravitational Wave} \\
	GW150914	& Binary black hole merger event detected on 14 September 2015 \\
	GW151226	& Binary black hole merger event detected on 26 December 2015 \\
	GW170104	& Binary black hole merger event detected on 4 January 2017 \\
	GW170814	& Binary black hole merger event detected on 14 August 2017 \\
	GW170817	& Binary neutron star merger event detected on 17 August 2017 \\
	\textit{INTEGRAL} & \emph{International Gamma-Ray Astrophysics Laboratory} \\
	LIGO	& \emph{Laser Interferometer Gravitational-Wave Observatory}, 4 km arm length interferometers in \\
	     &  in the US at Hanford WA and Livingston LA\\
	LIGO-India	& LIGO interferometer being built in India \\
	\textit{LISA}	& \emph{Laser Interferometer Space Antenna} \\
	NR	& \emph{Numerical Relativity} \\
	NS	& \emph{Neutron Star}\\
	NSBH	& \emph{Neutron Star--Black Hole}, a binary system of one neutron star and one black hole \\
	PM	& \emph{Post-Minkowskian} \\
	PNS	& \emph{Proto-Neutron Star} \\
	PN	& \emph{Post-Newtonian} \\
	QCD	& \emph{Quantum Chromodynamics} \\
	SASI	& \emph{Standing Accretion Shock Instability} \\
	SM	& the \emph{Standard Model} of particle physics \\
	SN, SNe	& \emph{Supernova}, \emph{Supernovae} \\
	SNR	& \emph{Signal-to-noise ratio} \\
    Virgo & 3 km arm length interferometer located in Cascina, Italy \\
	%\hline
        %\hline
	\end{tabular}
        }
        \end{tcolorbox}
        }
        \vskip-5pt
\end{table}  
\clearpage

